GRLinQ: An Intelligent Spectrum Sharing Mechanism for Device-to-Device Communications with Graph Reinforcement Learning

Device-to-device (D2D) spectrum sharing in wireless communications is a challenging non-convex combinatorial optimization problem, involving entangled link scheduling and power control in a large-scale network. The state-of-the-art methods, either from a model-based or a data-driven perspective, exhibit certain limitations such as the critical need for channel state information (CSI) and/or a large number of (solved) instances (e.g., network layouts) as training samples. To advance this line of research, we propose a novel hybrid model/datadriven spectrum sharing mechanism with graph reinforcement learning for link scheduling (GRLinQ), injecting information theoretical insights into machine learning models, in such a way that link scheduling and power control can be solved in an intelligent yet explainable manner. Through an extensive set of experiments, GRLinQ demonstrates superior performance to the existing model-based and data-driven link scheduling and/or power control methods, with a relaxed requirement for CSI, a substantially reduced number of unsolved instances as training samples, a possible distributed deployment, reduced online/offline computational complexity, and more remarkably excellent scalability and generalizability over different network scenarios and system configurations.

==> typeset_equations_v4.6/dot_emacs <==
;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;;; Copyright Stefan M. Moser
;;; 
;;; Version 1.0, 17 September 2004
;;; Version 1.1, 28 October 2004: changed IEEEeqnarray
;;; Version 2.0, 4 June 2006: improved IEEEeqnarray, linebreak, IEEEmulticol; 
;;;              added IEEEeqnarraystar
;;; Version 2.1, 30 March 2007: added linebreakwithoutspace, small corrections
;;; Version 3.0, 13 October 2008: removed \C-s and replaced by secure version 
;;;              that is independent of keyboard definitions
;;; Version 3.3, 29 March 2011: added \IEEElabel
;;; Version 3.5, 29 October 2011: worked over
;;; Version 4.0, 3 January 2013: removed IEEElabel
;;; Version 4.2, 6 August 2013: replace \: with \>
;;; Version 4.6, 29 September 2017: added \IEEEeqnarraylabel, \subnumberinglabel,
;;;              \IEEElabelanchoreqn
;;;
;;; You may change this code, but you always have to keep this 
;;; header (you may add to it).
;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;

;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; Add somewhere in your .emacs-file:

(fset 'IEEEeqnarray
   [?\\ ?b ?e ?g ?i ?n ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?} ?{ ?r ?C ?l ?} tab return return ?\\ ?e ?n ?d ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?} tab up tab])

(fset 'IEEEeqnarraystar
   [?\\ ?b ?e ?g ?i ?n ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?* ?} ?{ ?r ?C ?l ?} tab return return ?\\ ?e ?n ?d ?{ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?* ?} tab up tab])

(fset 'linebreak
   [?\\ ?n ?o ?n ?u ?m ?b ?e ?r ?\\ ?\\ tab return ?& ?& ?  right ?\\ ?> tab])

(fset 'linebreakwithoutspace
   [?\\ ?n ?o ?n ?u ?m ?b ?e ?r ?\\ ?\\ tab return ?& ?& ?  right tab])

(fset 'unlinebreak
   [?\C-\M-s ?\\ ?n ?o ?n ?u ?m ?b ?e ?r C-left left ?\C-  ?\C-\M-s ?& ?& right left ?\C-w])

(fset 'IEEEmulticol
   [?\C-a tab ?\\ ?I ?E ?E ?E ?e ?q ?n ?a ?r ?r ?a ?y ?m ?u ?l ?t ?i ?c ?o ?l ?{ ?3 ?} ?{ ?l ?} ?{ return tab escape ?x ?i ?s ?e ?a ?r ?c ?h ?- ?f ?o ?r ?w ?a ?r ?d return ?& left ?} ?\\ ?n ?o ?n ?u ?m ?b ?e ?r ?\\ ?\\ ?\\ ?q ?u ?a ?d return tab])


;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; Add the eight marked lines in the LaTeX-mode-hook, or if not 
;; existent, copy whole paragraph into your .emacs-file:
(require 'tex-site)
(setq LaTeX-mode-hook 
 '(lambda ()
    (define-key LaTeX-mode-map "\C-ci" 'IEEEeqnarray)         ;; add this line!
    (define-key LaTeX-mode-map "\C-co" 'IEEEeqnarraystar)     ;; add this line!
    (define-key LaTeX-mode-map "\C-cb" 'linebreak)            ;; add this line!
    (define-key LaTeX-mode-map "\C-cn" 'linebreakwithoutspace);; add this line!
    (define-key LaTeX-mode-map "\C-c\C-b" 'unlinebreak)       ;; add this line!
    (define-key LaTeX-mode-map "\C-cm" 'IEEEmulticol)         ;; add this line!
    (auto-fill-mode)
    (turn-on-reftex)
    (setq LaTeX-environment-list 
	  '(
	    (("abstract"))
	    (("array" LaTeX-env-array))
	    (("cases"))
	    (("center"))
	    (("claim" LaTeX-env-label))
	    (("conjecture" LaTeX-env-label))
	    (("corollary" LaTeX-env-label))
	    (("definition" LaTeX-env-label))
	    (("description" LaTeX-env-item))
	    (("document" LaTeX-env-document))
	    (("enumerate" LaTeX-env-item))
	    (("equation" LaTeX-env-label))
	    (("equation*"))
	    (("IEEEeqnarray" LaTeX-env-label))    ;; add this line!
	    (("IEEEeqnarray*"))                   ;; add this line!
	    (("example" LaTeX-env-label))
	    (("figure" LaTeX-env-figure))
	    (("figure*" LaTeX-env-figure))
		;(("filecontents" LaTeX-env-contents))
		;(("filecontents*" LaTeX-env-contents))
		;(("flushleft"))
		;(("flushright"))
	    (("itemize" LaTeX-env-item))
	    (("lemma" LaTeX-env-label))
	    (("list" LaTeX-env-list))
	    (("minipage" LaTeX-env-minipage))
	    (("multline" LaTeX-env-label))
	    (("multline*"))
	    (("picture" LaTeX-env-picture))
	    (("proposition" LaTeX-env-label))
	    (("quotation"))
	    (("quote"))
	    (("remark" LaTeX-env-label))
	    (("sloppypar"))
	    (("tabbing"))
	    (("table" LaTeX-env-figure))
	    (("table*" LaTeX-env-figure))
	    (("tabular" LaTeX-env-array))
	    (("tabular*" LaTeX-env-tabular*))
	    (("thebibliography" LaTeX-env-bib))
	    (("theindex" LaTeX-env-item))
	    (("theorem" LaTeX-env-label))
	    (("titlepage"))
	    (("trivlist" LaTeX-env-item))
	    (("verbatim"))
	    (("verbatim*"))
	    (("verse"))
	    )
	  )
))


;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; The following setting will make IEEEeqnarry/IEEEeqnarraybox known to
;; ispell: the spelling tool of Emacs.
;; Add the three marked lines to the ispell-tex-skip-alists in the corresponding
;; position, or if not existent, copy whole paragraph into your .emacs-file:
(setq ispell-local-dictionary "american")
(add-hook 'tex-mode-hook (function (lambda () (setq ispell-parser 'tex))))
(require 'ispell)
(setq ispell-tex-skip-alists
  '((
     ("%\\[" . "%\\]")
     ;; All the standard LaTeX keywords from L. Lamport's guide:
     ;; \cite, \hspace, \hspace*, \hyphenation, \include, \includeonly, \input,
     ;; \label, \nocite, \rule (in ispell - rest included here)
     ("\\\\addcontentsline"              ispell-tex-arg-end 2)
     ("\\\\psfrag"                       ispell-tex-arg-end-psfrag 0)
     ("\\\\add\\(tocontents\\|vspace\\)" ispell-tex-arg-end)
     ("\\\\\\([aA]lph\\|arabic\\)"       ispell-tex-arg-end)
     ("\\\\author"                       ispell-tex-arg-end)
     ("\\\\bibliographystyle"            ispell-tex-arg-end)
     ("\\\\bibliography"                 ispell-tex-arg-end)
     ("\\\\bstctlcite"                   ispell-tex-arg-end)
     ("\\\\eqref"                        ispell-tex-arg-end)
     ("\\\\thref"                        ispell-tex-arg-end)
     ("\\\\label"                        ispell-tex-arg-end)
     ("\\\\makebox"                      ispell-tex-arg-end 0)
     ("\\\\document\\(class\\|style\\)" .
      "\\\\begin[ \t\n]*{[ \t\n]*document[ \t\n]*}")
     )
    (;; delimited with \begin.  In ispell: displaymath, eqnarray, eqnarray*,
     ;; equation, minipage, picture, tabular, tabular* (ispell)
     ("\\(figure\\|table\\)\\*?"  ispell-tex-arg-end 0)
     ("list"                      ispell-tex-arg-end 2)
     ("IEEEeqnarray\\*?". "\\\\end[ \t\n]*{[ \t\n]*IEEEeqnarray\\*?[ \t\n]*}");; add this line!
     ("IEEEeqnarraybox[tm]?\\*?". "\\\\end[ \t\n]*{[ \t\n]*IEEEeqnarraybox[tm]?\\*?[ \t\n]*}");; add this line!
     ("program"         . "\\\\end[ \t\n]*{[ \t\n]*program[ \t\n]*}")
     ("verbatim\\*?"    . "\\\\end[ \t\n]*{[ \t\n]*verbatim\\*?[ \t\n]*}")
     ("gather\\*?"      . "\\\\end[ \t\n]*{[ \t\n]*gather\\*?[ \t\n]*}")
     )
))


;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;;
;; The following setting will make IEEEeqnarray known to reftex: the referencing 
;; tool of Emacs.  
;; Add the three marked lines to your reftex-label-alist, or if not
;; existent, copy whole paragraph into your .emacs-file:
(setq reftex-label-alist
 '(
   (nil              ?e "eq:"   "~\\eqref{%s}" nil nil)
   ("IEEEeqnarray"   ?e "eq:"   "~\\eqref{%s}" t   nil)          ;; add this line!
   ("IEEEeqnarray*"  ?e "eq:"   "~\\eqref{%s}" t   nil)          ;; add this line!
   ("\\IEEEeqnarraylabel{*}"      ?e "eq:"   "~\\eqref{%s}" t   nil) ;; add this line!
   ("\\subnumberinglabel{*}"      ?e "eq:"   "~\\eqref{%s}" t   nil) ;; add this line!
   ("\\IEEElabelanchoreqn{*}"     ?e "eq:"   "~\\eqref{%s}" t   nil) ;; add this line!
   ("lemma"          ?l "lem:"  "~\\ref{%s}"   t   ("lemma" "lem."))
   ("theorem"        ?h "thm:"  "~\\ref{%s}"   t   ("theorem" "th." "thm."))  
   ("corollary"      ?c "cor:"  "~\\ref{%s}"   t   ("corollary" "cor."))  
   ("conjecture"     ?j "conj:" "~\\ref{%s}"   t   ("conjecture" "conj."))  
   ("proposition"    ?p "prop:" "~\\ref{%s}"   t   ("proposition" "prop."))  
   ("claim"          ?m "clm:"  "~\\ref{%s}"   t   ("claim" "cl."))  
   ("definition"     ?d "def:"  "~\\ref{%s}"   t   ("definition" "def."))  
   ("remark"         ?r "rem:"  "~\\ref{%s}"   t   ("remark" "rem."))  
   ("example"        ?x "ex:"   "~\\ref{%s}"   t   ("example" "ex."))  
   ("exercise"       ?x "ex:"   "~\\ref{%s}"   t   ("exercise" "exer." "exerc." "ex."))  
   ("enumerate"      ?i "item:" "~\\ref{%s}"   t   ("part"))  
   ))


